Stability in Single-Peaked Strategic Resource Selection Games

The strategic selection of resources by selfish agents has long been a key area of research, with Resource Selection Games and Congestion Games serving as prominent examples. In these traditional frameworks, agents choose from a set of resources, and their utility depends solely on the number of other agents utilizing the same respective resource, treating all agents as indistinguishable or anonymous. Only recently, the study of the Resource Selection Game with heterogeneous agents has begun, meaning agents have a type and the fraction of agents of their type at their resource is the basis of their decision-making. In this work, we initiate the study of the Resource Selection Game with heterogeneous agents in combination with single-peaked utility functions, as some research suggests that this may represent human decision-making in certain cases. We conduct a comprehensive analysis of the game's stability within this framework. We provide tight bounds that specify for which peak values equilibria exist across different dynamics on cycles and binary trees. On arbitrary graphs, in a setting where agents lack information about the selection of other agents, we provide tight bounds for the existence of equilibria, given that the utility function is linear on both sides of the peak. Agents possessing this information on arbitrary graphs creates the sole case where our bounds are not tight, instead, we narrow down the cases in which the game may admit equilibria and present how several conventional approaches fall short in proving stability.

==> Preliminaries/model.tex <==
We consider a strategic game, called the \emph{Resource Selection Game} played on a bipartite \emph{accessibility graph} $\G = (\res \cup \act, \edg)$, where $\res \cap \act = \emptyset$, $\res$ is the set of \emph{resources} and $\act$ is the set of \emph{agents}. A resource $q \in \res$ can be used by an agent $a \in \act$ if and only if $\{q,a\} \in \edg$ and may be used by any number of agents at the same time. We use the short hands $|\act|=n$ and $|\res|=k$.\\

Every agent in the Resource Selecction Game is either \emph{red} or \emph{blue}. For the set of red agents $\red$ and the set of blue agents $\blue$ it holds that $\red \cup \blue = \act$ and $\red \cap \blue = \emptyset$. We denote $|\red|=r$ and $|\blue|=b$.\\

Formally, for an agent $a$ we denote their \emph{accessible resources} with $Q(a)\subseteq \res$. Similarly $A(q)$ defines the agents, who have access to the resource $q$. We call $deg_G(a)=|Q(a)|$ the \emph{degree} of $a$ and $deg_G(q)=|A(q)|$ the \emph{degree} of $q$. As a shorthand for the \emph{maximum degree of any resource in $G$} we use $\Delta_G(\res)=max_{q\in\res}(deg_G(q))$. The selected resource of any agent $a$ in a given step is denoted by $\bold{s}(a)$ and is called $a$'s \emph{strategy}. The vector of all agent's strategies $\bold{s}=(\bold{s}(a_1),\bold{s}(a_2),...,\bold{s}(a_n)))$, with $a_i\in\act$ and $\bold{s}(a_i)\in Q(\bold{s}(a_i))$ for $i\in[1,n]$ is called \emph{strategy profile}. The number of agents at a given resource in a given strategy profile is denoted by $\#(q,\bold{s})=|\{a\in \act|\bold{s}(a) = q\}|$. Similarly we define $\#_R(q,\bold{s})=|\{a\in \red|\bold{s}(a) = q\}|$ and $\#_B(q,\bold{s})=|\{a\in\blue|\bold{s}(a) = q\}|$. We call the 2-tuple $(\#_R(q,\strat),\#_B(q,\strat))$ the \emph{state} of $q$. We notate resource \emph{state transitions} with an arrow from the initial state towards the new state in the color of the agent, who joined or left the resource to cause the state transition (e.g. \color{red} 1 \color{blue} 1 \color{red} -> 2 \color{blue} 1 \color{black} visualizes the state transition of a resource with one blue and one red agent, when a red agent joins). As a shorthand for a resource changing its state and then changing again to return to its initial state we use a double-headed arrow (e.g. \color{red} 1 \color{blue} 1 \color{red} <-> 2 \color{blue} 1 \color{black} to visualize a resource oscillating between a state with one or two red agents and one blue agent because of alternating joins and leaves by red agents). \\

Additionally, $\rho_R(q,\bold{s}) = \frac{\#_R(q,\bold{s})}{\#(q,\bold{s})}$ and
$\rho_B(q,\bold{s}) = \frac{\#_B(q,\bold{s})}{\#(q,\bold{s})}$ denote the fraction of red or blue agents at $q$ in $\bold{s}$. We note that these functions are undefined for empty resources (where $\#(q,\strat)=0$). If either $\#_R(q,\strat)=0$ or $\#_B(q,\strat)=0$ holds we call $q$ \emph{monochromatic}. In particular, if $q$ is monochromatic in $\strat$ and $\#(q,\strat)=m$, we call q \emph{m-monochromatic}. We call a resource, which is not empty and not monochromatic \emph{polychromatic}.
\\
 An agents \emph{utility} is its satisfaction at a given resource in a given strategy profile. We diverge from the Schelling Resource Selection Game in that agents are not necessarily homophilic. Instead, agents prefer a fraction $\Lambda \in (0,1)$ of agents of their color at their resource. The utility of an agent then decreases linearly with the fraction of agents of the same color moving further away from $\Lambda$ in either direction. Because of these properties we call the function to determine the agents utility in our model \emph{single peaked} (around $\Lambda$). To formally define this function we first define the following function.
\begin{restatable}[$p$]{definition}{definition_p}
    The function $p$ has exactly one peak at some fraction $\Lambda \in (0,1)$. Additionally, every valid instantiation of $p$ has to fulfill the following properties
    \begin{itemize}
        \item $p$ is monotonically increasing in $[0,\Lambda]$ with $p(0)=0$
        \item for all $x \in (\Lambda,1]$ $p(x) = p(\frac{\Lambda(1-x)}{1-\Lambda})$.
    \end{itemize}
    Note that for all $x \in (\Lambda,1]$, it holds that $\frac{\Lambda(1-x)}{1-\Lambda}\in[0,\Lambda]$ \footnote[-0,2][0]{The statement follows directly from transforming the assumption:
       \begin{equation*} 
           x>\Lambda \iff \frac{1}{1-x}>\frac{1}{1-\Lambda} \iff \frac{\Lambda}{1-x}>\frac{\Lambda}{1-\Lambda} \iff \Lambda>\frac{\Lambda(1-x)}{1-\Lambda}.
       \end{equation*}} 
   and thus $p(x)\leq\Lambda$. \
\end{restatable}

Using $p$ we now can define the \emph{utility function} $u$. 
\begin{restatable}[utility function]{definition}{definition_utility_function}
    Let $a\in\act$ and $\strat$ be a strategy profile. Then
        \[ 
    u(a,\bold{s})= \left\{
    \begin{array}{ll} 
        \label{def:p}
          p(\rho_R(\bold{s}(a))) & \text{if } a \in \red \\
          p(\rho_B(\bold{s}(a))) & \text{if } a \in \blue\\
    \end{array} 
    \right. 
    \]
    is $a$'s utility in $\strat$.
\end{restatable}
For a strategy profile $\bold{s}$ with $\bold{s}(a_i) = q$, we use the shorthand $\bold{s} = (q,\bold{s_{-i}})$, where $\bold{s_{-i}} = (\bold{s}(a_1),…\bold{s}(a_{i-1}),\bold{s}(a_{i+1}),…,\bold{s}(a_n))$ is identical to $\bold{s}$ without the i-th entry. The \emph{social welfare} of a strategy profile $\strat$ is the sum of all agents' utilities in $\strat$, formally defined as $W(\strat)=\sum_{a\in\act}u(a,\strat)$. Moreover, to denote the social welfare at a specific resource $q\in\res$ within the strategy profile $\strat$ at $q\in\res$, we write $W_q(\strat)$.

Additionally, we differentiate between \emph{impact-blind} and \emph{impact-aware} agents. Let $\bold{s'}=(q',\bold{s}_{-i})$ be the result of the jump of agent $i$ from resource $q$ to $q'$, with everything else staying the same, i.e. $\bold{s}(a_j)=\bold{s'}(a_j)$ if and only if $j\neq i$. We call the strategy change from $\bold{s}$ to $\bold{s'}$ an impact-aware improving move for an agent $a_i$ if $u(a_i,(q',\bold{\strat'})) > u(a_i,(q,\bold{s}))$. Meanwhile, an impact-blind improving move for a w.l.o.g. red agent $a_i$ is a strategy change, where $p(\rho_R(q',\bold{s}))>u(a_i,\bold{s})$. The impact-blindness models a lack of of knowledge of agents about the strategy of the other agents, in that while they know the fraction of their type at any resource, they are unaware of how their jump will alter that fraction. We note that in our model in the impact-blind setting agents never jump to empty resources as for $q\in\res$ with $A(q)=\emptyset$ and a strategy profile $\strat$ the utility they see $p(\rho_R(q,\strat))$ would be undefined. This is in accordance with \autoref{def:p} as $p(0)=0$. We see that a similar statement holds for the impact-aware setting.
\begin{restatable}[]{lemma}{IA_no_jumps_to_empty}
    In the impact-aware setting agents do not jump to empty resources.
\end{restatable}

\begin{proof}
    Let $q'$ with $A(q')=\emptyset$. For a jump by an agent $a\in\act$ from a resource $q\in\res$ to $q'\in\res$, changing the strategy profile from $\strat$ to $\strat'$, it holds that $u(a,(q',\strat'))=p(1)=0\leq u(a,\strat)$ and thus the move is not impact-aware improving.
\end{proof}

We further note that an impact-aware improving move may not be an impact-blind improving move. \footnote[-0,2][0]{For $\Lambda=\frac{1}{2}$ let a red agent $a$ jump from a resource $q$ to $q'$, altering the strategy profile from $\strat$ to $\strat'$, with $u(a,\strat)=p(\frac{2}{5})$, $\#_R(q',\strat)=1$ and $\#_B(q',\strat)=2$. Then it holds that $p(\rho_R(q',\strat))<u(a,\strat)<u(a,\strat')$.}

Furthermore, deviating from the Schelling Resource Selection Game, an impact-blind improving move may not be impact-aware improving. \footnote[-0,2][0]{To see this, let $\Lambda=\frac{1}{2}$ and let a red agent $a$ jump from a resource $q$ to $q'$, altering the strategy profile from $\strat$ to $\strat'$, with $u(a,\strat)=p(\frac{2}{5})$, $\#_R(q',\strat)=1$ and $\#_B(q',\strat)=1$. Then it holds that $p(\rho_R(q',\strat))>u(a,\strat)>u(a,\strat')$.}

Based on impact-aware and impact-blind improving moves, we define two states of strategy profiles. We say a strategy profile $\strat$ is in \emph{impact-aware-equilibrium} (\emph{IAE}), if no agent has an impact-aware improving move they wish to make. Similarly a strategy profile $\strat$ is in \emph{impact-blind-equilibrium} (\emph{IBE}), if no agent has an impact-blind improving move they wish to make.

We say that a game in which agents only make impact-blind improving moves has \emph{impact-blind dynamics} and a game in which agents only perform impact-aware improving moves has \emph{impact-aware dynamics}. In a game with impact-blind dynamics, the \emph{IB-FIP} (\emph{impact-blind finite improvement property}) holds if and only if from every strategy profile an IBE is reached after a finite number of steps. We define the \emph{IA-FIP} analogously.

Note, that we only consider unilateral moves, meaning agents can change its strategy without the consent of other agents being necessary.

\\
